HammingMesh: A Network Topology for Large-Scale Deep Learning

Numerous microarchitectural optimizations unlocked tremendous processing power for deep neural networks that in turn fueled the AI revolution. With the exhaustion of such optimizations, the growth of modern AI is now gated by the performance of training systems, especially their data movement. Instead of focusing on single accelerators, we investigate data-movement characteristics of large-scale training at full system scale. Based on our workload analysis, we design HammingMesh, a novel network topology that provides high bandwidth at low cost with high job scheduling flexibility. Specifically, HammingMesh can support full bandwidth and isolation to deep learning training jobs with two dimensions of parallelism. Furthermore, it also supports high global bandwidth for generic traffic. Thus, HammingMesh will power future large-scale deep learning systems with extreme bandwidth requirements.

==> Makefile <==
DOCUMENT=$(shell ls -1 *tex | sed -e "s/\.tex//")

FILES=*.tex 

all: $(DOCUMENT).pdf

$(DOCUMENT).pdf: $(FILES)
	if [ -f plt/Makefile ]; then make -C plt; fi
	if [ -f img/Makefile ]; then make -C img; fi
	if [ -d ../img ]; then make -C ../img; fi
	rm -f pdflatex.out
#	cd ppt && sh ./crop_all.sh
	pdflatex --shell-escape $(DOCUMENT).tex 2>&1 | tee pdflatex.out
	if grep -q citation $(DOCUMENT).aux; then bibtex $(DOCUMENT); fi;
# don't use pdflatex due to transparency issues  
	pdflatex --shell-escape $(DOCUMENT).tex 2>&1 | tee pdflatex.out
	pdflatex --shell-escape $(DOCUMENT).tex 2>&1 | tee pdflatex.out
	#dvips $(DOCUMENT).dvi -o $(DOCUMENT).ps
# use ps2pdf to avoid lossy image compression in pdf which looks ugly on the
# beamer
	#ps2pdf14 -dPDFSETTINGS=/printer -dAutoFilterColorImages=false -dColorImageFilter=/FlateEncode $(DOCUMENT).ps

copyin: ~/projekte/latex/macros/*
	cp ~/projekte/latex/macros/bibliography.bib .
	cp ~/projekte/latex/macros/htor.sty .
	cp ~/projekte/latex/macros/htor_paper.cls .

show: $(DOCUMENT).pdf
	atril $(DOCUMENT).pdf

spell:
	ln -sf ~/projekte/templates/aspell.en_US.dic .
	for i in $$(ls -1 *.tex); do \
		echo "checking $$i ... "; \
		aspell -t --lang=en_US --home-dir="$$(pwd)" -p aspell.en_US.dic -c $$i; \
done; \

force:
	touch $(DOCUMENT).tex
	make $(DOCUMENT).pdf

clean:
	if [ -f plt/Makefile ]; then make -C plt clean; fi
	rm -f *.aux *.out sparsity.synctex.gz
	rm -f $(DOCUMENT).blg $(DOCUMENT).dvi $(DOCUMENT).vrb $(DOCUMENT).bbl comment.cut 
	rm -f $(DOCUMENT).pdf $(DOCUMENT).toc $(DOCUMENT).lo[a,f,g,h,l,t]
	rm -f $(DOCUMENT).nav $(DOCUMENT).snm $(DOCUMENT).ps $(DOCUMENT).out
	rm -f aspell*dic
	if [ -f plt/Makefile ]; then make -C plt clean; fi
	if [ -d img ]; then make -C img clean; fi
	if [ -d slides ]; then make -C img clean; fi
	if [ -d ../img ]; then make -C ../img clean; fi

pack: $(DOCUMENT).tgz

$(DOCUMENT).tgz: *.tex
	mkdir $(DOCUMENT) 
	cp *.tex $(DOCUMENT)
	cp *.sty $(DOCUMENT)
	cp *.cls $(DOCUMENT)
	cp *.bib $(DOCUMENT)
	if [ -d img ]; then cp -a img $(DOCUMENT); fi
	if [ -d kivio ]; then cp -a kivio $(DOCUMENT); fi
	cp Makefile $(DOCUMENT)
	make -C $(DOCUMENT)
	cp $(DOCUMENT)/$(DOCUMENT).pdf $(DOCUMENT)/$(DOCUMENT)_orig.pdf
	make -C $(DOCUMENT) clean
	tar czf $(DOCUMENT).tgz $(DOCUMENT) --exclude=.svn 
	tar tzf $(DOCUMENT).tgz
	rm -fr $(DOCUMENT)
	@echo "voila: $(DOCUMENT).tgz"

commit: clean 
	svn commit

count: $(DOCUMENT).pdf
	pdftotext $(DOCUMENT).pdf -|wc -w

update: clean 
	svn update


